The Gemini NICI Planet-Finding Campaign: The Frequency of Giant Planets Around Debris Disk Stars

We have completed a high-contrast direct imaging survey for giant planets around 57 debris disk stars as part of the Gemini NICI Planet-Finding Campaign. We achieved median H-band contrasts of 12.4 mag at 0.5" and 14.1 mag at 1" separation. Follow-up observations of the 66 candidates with projected separation < 500 AU show that all of them are background objects. To establish statistical constraints on the underlying giant planet population based on our imaging data, we have developed a new Bayesian formalism that incorporates (1) non-detections, (2) single-epoch candidates, (3) astrometric and (4) photometric information, and (5) the possibility of multiple planets per star to constrain the planet population. Our formalism allows us to include in our analysis the previously known Beta Pictoris and the HR 8799 planets. Our results show at 95% confidence that <13% of debris disk stars have a >5MJup planet beyond 80 AU, and <21% of debris disk stars have a >3MJup planet outside of 40 AU, based on hot-start evolutionary models. We model the population of directly-imaged planets as d^2N/dMda ~ m^alpha a^beta, where m is planet mass and a is orbital semi-major axis (with a maximum value of amax). We find that beta < -0.8 and/or alpha > 1.7. Likewise, we find that beta < -0.8 and/or amax < 200 AU. If we ignore the Beta Pic and HR 8799 planets (should they belong to a rare and distinct group), we find that < 20% of debris disk stars have a > 3MJup planet beyond 10 AU, and beta < -0.8 and/or alpha < -1.5. Our Bayesian constraints are not strong enough to reveal any dependence of the planet frequency on stellar host mass. Studies of transition disks have suggested that about 20% of stars are undergoing planet formation; our non-detections at large separations show that planets with orbital separation > 40 AU and planet masses > 3 MJup do not carve the central holes in these disks.

==> cands_table.tex <==
\begin{deluxetable}{lrrrrrrr}
\tabletypesize{\scriptsize}
\tablecaption{Follow-up NICI Astrometry}
\tablewidth{0pt}
\tablehead{ \colhead{Target}  &\colhead{Obj. No.} &\colhead{Epoch} & \colhead{Sep.($''$)} & \colhead{Sep. Unc. ($''$)} & \colhead{PA (deg)} & \colhead{PA Unc. (deg)} & \colhead{$\Delta H$ (mag)}}
\startdata
HD 19668 &  1 &       2010.66 &   5.470 &   0.009 &   150.5 &   0.2 &  11.8 \\
 &  1 &       2010.98 &   5.415 &   0.009 &   150.8 &   0.2 &  11.8 \\
 &  1 &       2011.70 &   5.320 &   0.009 &   151.4 &   0.2 &  11.8 \\
HD 27290 &  1 &       2008.96 &   7.745 &   0.009 &   244.0 &   0.2 &  12.8 \\
 &  1 &       2010.01 &   7.914 &   0.009 &   242.3 &   0.2 &  12.8 \\
HD 31295 &  1 &       2009.04 &   6.256 &   0.009 &   271.6 &   0.2 &  15.5 \\
 &  1 &       2010.98 &   6.368 &   0.009 &   273.9 &   0.2 &  15.5 \\
 &  2 &       2009.04 &   8.810 &   0.009 &   316.6 &   0.2 &  16.8 \\
 &  2 &       2010.98 &   9.050 &   0.009 &   317.2 &   0.2 &  16.8 \\
$\zeta$ Lep &  1 &       2008.95 &   5.302 &   0.009 &   110.0 &   0.2 &  20.7
 \\
 &  1 &       2011.20 &   5.390 &   0.009 &   109.6 &   0.2 &  20.7 \\
HD 54341 &  1 &       2008.95 &   3.078 &   0.009 &   130.8 &   0.2 &  14.9 \\
 &  1 &       2010.98 &   3.077 &   0.009 &   131.9 &   0.2 &  14.9 \\
 &  2 &       2008.95 &   4.359 &   0.009 &   137.1 &   0.2 &  14.3 \\
 &  2 &       2010.98 &   4.363 &   0.009 &   137.9 &   0.2 &  14.3 \\
HD 61005 &  1 &       2009.03 &   3.581 &   0.009 &   326.5 &   0.2 &  14.8 \\
 &  1 &       2011.31 &   3.340 &   0.009 &   326.4 &   0.2 &  14.8 \\
 &  2 &       2009.03 &   6.381 &   0.009 &   315.2 &   0.2 &  14.4 \\
 &  2 &       2011.31 &   6.142 &   0.009 &   314.6 &   0.2 &  14.4 \\
 &  3 &       2009.03 &   7.171 &   0.009 &   191.6 &   0.2 &  14.9 \\
 &  3 &       2011.31 &   7.309 &   0.009 &   190.0 &   0.2 &  14.9 \\
HD 71155 &  1 &       2008.96 &   5.770 &   0.009 &    86.7 &   0.2 &  17.0 \\
 &  1 &       2011.37 &   5.955 &   0.009 &    86.2 &   0.2 &  17.0 \\
 &  2 &       2008.96 &   9.410 &   0.009 &   246.1 &   0.2 &  16.7 \\
 &  2 &       2011.37 &   9.229 &   0.009 &   245.5 &   0.2 &  16.7 \\
TWA 7 &  1 &       2009.11 &   3.203 &   0.009 &   121.3 &   0.2 &  10.5 \\
 &  1 &       2010.16 &   3.316 &   0.009 &   119.5 &   0.2 &  10.5 \\
 &  2 &       2009.11 &   3.931 &   0.009 &    92.4 &   0.2 &  16.4 \\
 &  2 &       2010.16 &   4.072 &   0.009 &    92.0 &   0.2 &  16.4 \\
 &  3 &       2009.11 &   4.948 &   0.009 &   172.8 &   0.2 &  15.7 \\
 &  3 &       2010.16 &   4.953 &   0.009 &   170.9 &   0.2 &  15.7 \\
HD 138965 &  1 &       2009.12 &   1.716 &   0.009 &    61.3 &   0.2 &  11.2 \\
 &  1 &       2011.32 &   1.845 &   0.009 &    59.7 &   0.2 &  11.2 \\
 &  2 &       2009.12 &   4.089 &   0.009 &   244.7 &   0.2 &  14.5 \\
 &  2 &       2011.32 &   3.931 &   0.009 &   245.8 &   0.2 &  14.5 \\
 &  3 &       2009.12 &   7.381 &   0.009 &   157.3 &   0.2 &  12.9 \\
 &  3 &       2011.32 &   7.300 &   0.009 &   155.9 &   0.2 &  12.9 \\
 &  4 &       2009.12 &   7.511 &   0.009 &   102.1 &   0.2 &  14.9 \\
 &  4 &       2011.32 &   7.597 &   0.009 &   100.9 &   0.2 &  14.9 \\
 &  5 &       2009.12 &   7.832 &   0.009 &   236.4 &   0.2 &  12.0 \\
 &  5 &       2011.32 &   7.683 &   0.009 &   236.9 &   0.2 &  12.0 \\
 &  6 &       2009.12 &   8.041 &   0.009 &   327.0 &   0.2 &  13.1 \\
 &  6 &       2011.32 &   8.112 &   0.009 &   327.8 &   0.2 &  13.1 \\
 &  7 &       2009.12 &   9.971 &   0.009 &     4.3 &   0.2 &  15.5 \\
 &  7 &       2011.32 &  10.085 &   0.009 &     4.6 &   0.2 &  15.5 \\
$\gamma$ Oph &  1 &       2009.19 &   4.528 &   0.018 &    59.2 &   0.5 &  15.7
 \\
 &  1 &       2010.27 &   4.588 &   0.018 &    58.5 &   0.5 &  15.7 \\
 &  2 &       2009.19 &   5.902 &   0.018 &   239.4 &   0.5 &  17.1 \\
 &  2 &       2010.27 &   5.837 &   0.018 &   240.0 &   0.5 &  17.1 \\
 &  3 &       2009.19 &   6.210 &   0.018 &   267.3 &   0.5 &  13.9 \\
 &  3 &       2010.27 &   6.183 &   0.018 &   268.2 &   0.5 &  13.9 \\
 &  4 &       2009.19 &   6.602 &   0.018 &   275.0 &   0.5 &  16.2 \\
 &  4 &       2010.27 &   6.589 &   0.018 &   275.8 &   0.5 &  16.2 \\
 &  5 &       2009.19 &   6.964 &   0.018 &    59.1 &   0.5 &  14.9 \\
 &  5 &       2010.27 &   7.032 &   0.018 &    58.8 &   0.5 &  14.9 \\
 &  6 &       2009.19 &   8.677 &   0.018 &    96.3 &   0.5 &  13.6 \\
 &  6 &       2010.27 &   8.707 &   0.018 &    95.1 &   0.5 &  13.6 \\
 &  7 &       2009.19 &   9.271 &   0.018 &   253.6 &   0.5 &  16.9 \\
 &  7 &       2010.27 &   9.229 &   0.018 &   254.1 &   0.5 &  16.9 \\
HD 170773 &  1 &       2011.79 &   4.591 &   0.009 &   232.4 &   0.2 &  17.5 \\
 &  1 &       2012.26 &   4.638 &   0.009 &   233.2 &   0.2 &  17.5 \\
 &  2 &       2011.79 &   4.751 &   0.009 &   219.9 &   0.2 &  17.7 \\
 &  2 &       2012.26 &   4.785 &   0.009 &   220.8 &   0.2 &  17.7 \\
 &  3 &       2011.79 &   4.793 &   0.009 &    96.4 &   0.2 &  17.4 \\
 &  3 &       2012.26 &   4.706 &   0.009 &    96.1 &   0.2 &  17.4 \\
 &  4 &       2011.79 &   6.899 &   0.009 &   113.6 &   0.2 &  14.6 \\
 &  4 &       2012.26 &   6.807 &   0.009 &   113.6 &   0.2 &  14.6 \\
 &  5 &       2011.79 &   7.575 &   0.009 &    51.9 &   0.2 &  14.5 \\
 &  5 &       2012.26 &   7.521 &   0.009 &    51.2 &   0.2 &  14.5 \\
 &  5 &       2011.36 &   7.551 &   0.009 &    51.7 &   0.2 &  14.5 \\
 &  6 &       2011.79 &   7.684 &   0.009 &    44.6 &   0.2 &  17.5 \\
 &  6 &       2012.26 &   7.648 &   0.009 &    43.8 &   0.2 &  17.5 \\
 &  7 &       2011.79 &   7.802 &   0.009 &   327.9 &   0.2 &  16.6 \\
 &  7 &       2012.26 &   7.860 &   0.009 &   327.2 &   0.2 &  16.6 \\
 &  8 &       2011.79 &   7.866 &   0.009 &   343.8 &   0.2 &  14.7 \\
 &  8 &       2012.26 &   7.900 &   0.009 &   343.1 &   0.2 &  14.7 \\
 &  9 &       2011.79 &   7.879 &   0.009 &   161.1 &   0.2 &  14.8 \\
 &  9 &       2012.26 &   7.816 &   0.009 &   161.5 &   0.2 &  14.8 \\
 & 10 &       2011.79 &   7.921 &   0.009 &   337.3 &   0.2 &  17.4 \\
 & 10 &       2012.26 &   7.962 &   0.009 &   336.5 &   0.2 &  17.4 \\
 & 11 &       2011.79 &   7.964 &   0.009 &   141.5 &   0.2 &  15.1 \\
 & 11 &       2012.26 &   7.874 &   0.009 &   141.8 &   0.2 &  15.1 \\
 & 12 &       2011.79 &   8.262 &   0.009 &   263.9 &   0.2 &  17.1 \\
 & 12 &       2012.26 &   8.354 &   0.009 &   264.0 &   0.2 &  17.1 \\
 & 12 &       2011.36 &   8.278 &   0.009 &   263.4 &   0.2 &  17.1 \\
 & 13 &       2011.79 &   8.490 &   0.009 &   213.2 &   0.2 &  17.4 \\
 & 13 &       2012.26 &   8.504 &   0.009 &   213.7 &   0.2 &  17.4 \\
 & 13 &       2011.36 &   8.524 &   0.009 &   212.9 &   0.2 &  17.4 \\
 & 14 &       2011.79 &   9.150 &   0.009 &   313.7 &   0.2 &  16.2 \\
 & 14 &       2012.26 &   9.225 &   0.009 &   313.2 &   0.2 &  16.2 \\
 & 15 &       2011.79 &   9.696 &   0.009 &   245.3 &   0.2 &  16.3 \\
 & 15 &       2012.26 &   9.764 &   0.009 &   245.6 &   0.2 &  16.3 \\
 & 16 &       2011.79 &  10.030 &   0.009 &   265.4 &   0.2 &  14.3 \\
 & 16 &       2011.36 &  10.051 &   0.009 &   264.9 &   0.2 &  14.3 \\
 & 16 &       2012.26 &  10.129 &   0.009 &   265.4 &   0.2 &  14.3 \\
 & 17 &       2012.26 &  10.424 &   0.009 &   136.7 &   0.2 &  14.4 \\
 & 17 &       2011.36 &  10.513 &   0.009 &   136.5 &   0.2 &  14.4 \\
 & 18 &       2011.79 &  11.722 &   0.009 &   184.5 &   0.2 &  14.6 \\
 & 18 &       2011.36 &  11.752 &   0.009 &   184.3 &   0.2 &  14.6 \\
HD 176638 &  1 &       2011.79 &   3.508 &   0.009 &   157.8 &   0.2 &  18.0 \\
 &  1 &       2012.26 &   3.473 &   0.009 &   158.8 &   0.2 &  18.0 \\
 &  2 &       2011.36 &   4.732 &   0.009 &    93.5 &   0.2 &  14.4 \\
 &  2 &       2011.79 &   4.732 &   0.009 &    93.3 &   0.2 &  14.4 \\
 &  2 &       2012.26 &   4.660 &   0.009 &    93.4 &   0.2 &  14.4 \\
 &  3 &       2011.79 &   5.231 &   0.009 &   265.7 &   0.2 &  18.2 \\
 &  3 &       2012.26 &   5.293 &   0.009 &   265.7 &   0.2 &  18.2 \\
 &  4 &       2011.79 &   9.409 &   0.009 &   319.6 &   0.2 &  18.1 \\
 &  4 &       2011.36 &   9.359 &   0.009 &   319.4 &   0.2 &  18.1 \\
 &  4 &       2012.26 &   9.420 &   0.009 &   319.4 &   0.2 &  18.1 \\
HD 53143 &  1 &      2009.04 &   4.540 &   0.009 &   -74.4 &   0.2 &  12.0 \\
                 &  1 &      2010.01 &   4.304 &   0.009 &   -77.4 &   0.2 &  12.0 \\
HD 107146 &  1 &      2009.04 &   6.78 &   0.009 &   -142.7 &   0.2 &  16.5 \\
                   &  1 &      2010.27 &   6.50 &   0.009 &   -143.4 &   0.2 &  16.5 \\
\enddata
\label{tab:cands}
\end{deluxetable}


==> mass_sep_constraints.tex <==
\begin{deluxetable}{c|rrrr}
\tabletypesize{\scriptsize}
\tablecaption{Debris Disk Stars Observed by Campaign.}
\tablewidth{0pt}
\tablehead{ \colhead{} &\colhead{0.5--3~\mjup } & \colhead{3--6~\mjup  } & \colhead{6--9~\mjup  } & \colhead{9--13~\mjup  }}
\startdata
0.5--3~AU &   0.84 &   0.87 &   0.88 &   0.94 \\
3--15~AU  &   0.42 &   0.43 &   0.44 &   0.53 \\
15-75~AU  &   0.31 &   0.16 &   0.16 &   0.21 \\
75--500~AU &   0.09 &   0.07 &   0.06 &   0.08 \\
\enddata
\label{tab:obs}
\end{deluxetable}


==> mass_table.tex <==
\begin{deluxetable}{lcccccc}
\tabletypesize{\scriptsize}
\tablecaption{Lowest mass companion detectable at different projected separations (\mjup).}
\tablewidth{0pt}
\tablehead{ \colhead{Target} &\colhead{0.5$''$} & \colhead{1$''$} & \colhead{2$''$} & \colhead{4$''$} & \colhead{8$''$} & \colhead{at outer disk}}
\startdata
\enddata
\label{tab:contrasts}
\tablecomments{The last column gives the lowest mass companion detectable at the outer radius of the debris disk.}
\end{deluxetable}

==> obs_table_oct24_2012.tex <==
\begin{deluxetable}{lcrrrr}
\tabletypesize{\scriptsize}
\tablecaption{Observation of Campaign Debris-Disk Targets}
\tablewidth{0pt}
\tablehead{ \colhead{Target}  &\colhead{Date} & \colhead{Obs Mode} & \colhead{Nunber of} & \colhead{Total}             & \colhead{Total} \\
                   \colhead{}           & \colhead{}        &\colhead{}                  & \colhead{Images}     & \colhead{Exp. Time (s)} & \colhead{Rotation (deg)} 
}
\startdata
HR 9 & 2009-12-05 & ADI &      20 &    1208 &     2.8 \\
HR 9 & 2009-12-05 & ASDI &      45 &    2736 &    22.8 \\
49 Cet & 2009-12-02 & ASDI &      45 &    2736 &    40.6 \\
49 Cet & 2009-12-02 & ADI &      20 &    1208 &    16.4 \\
HD 10939 & 2010-12-26 & ASDI &      44 &    2708 &     3.5 \\
HIP 10679 & 2011-10-16 & ASDI &      45 &    2701 &    13.3 \\
HD 15115 & 2009-12-04 & ADI &      20 &    1208 &     6.2 \\
HD 15115 & 2009-12-04 & ASDI &      43 &    2598 &    17.4 \\
HD 15115 & 2011-11-07 & ADI &      20 &    1185 &     8.6 \\
HD 15115 & 2011-11-22 & ADI &      40 &    2371 &    13.7 \\
HD 17848 & 2008-12-16 & ADI &      20 &    1200 &     9.7 \\
HD 17848 & 2008-12-16 & ASDI &      45 &    2650 &    22.3 \\
HD 19668 & 2010-08-29 & ADI &      20 &    1208 &     9.1 \\
HD 19668 & 2010-08-29 & ASDI &      45 &    2701 &    30.6 \\
HD 21997 & 2009-01-16 & ASDI &      45 &    2530 &    55.6 \\
HD 21997 & 2009-01-16 & ADI &      20 &    1208 &     3.6 \\
HD 21997 & 2010-01-09 & ADI &      20 &    1208 &     0.8 \\
HD 21997 & 2010-10-31 & ASDI &      50 &    3021 &    89.2 \\
HD 21997 & 2010-12-25 & ASDI &      27 &    1631 &  -233.9 \\
Eps Eri & 2009-12-03 & ADI &      60 &    3556 &    18.6 \\
Eps Eri & 2009-12-03 & ASDI &      60 &    3556 &    18.5 \\
Eps Eri & 2011-10-16 & ASDI &     180 &    3693 &    55.7 \\
Eps Eri & 2011-10-16 & ASDI &     180 &    3693 &    55.8 \\
Eps Eri & 2011-10-16 & ASDI &     180 &    3693 &     1.9 \\
HD 24966 & 2009-01-15 & ADI &      20 &    1208 &    17.1 \\
HD 24966 & 2009-01-15 & ASDI &      48 &    2699 &    72.3 \\
HD 25457 & 2009-01-13 & ASDI &      44 &    2489 &    25.5 \\
HD 25457 & 2009-01-13 & ADI &      20 &    1208 &     8.5 \\
HD 27290 & 2008-12-18 & ADI &      20 &    1185 &    13.3 \\
HD 27290 & 2008-12-18 & ASDI &      45 &    2565 &    37.0 \\
HD 27290 & 2010-01-05 & ADI &      45 &    2667 &    14.5 \\
HD 31295 & 2009-01-14 & ASDI &      45 &    2616 &    16.4 \\
HD 31295 & 2009-01-14 & ADI &      20 &    1208 &     8.0 \\
HD 32297 & 2008-12-17 & ADI &      20 &    1200 &     4.5 \\
HD 32297 & 2008-12-17 & ASDI &      45 &    2701 &    14.1 \\
HIP 25486 & 2009-01-14 & ASDI &      45 &    2479 &    34.6 \\
HIP 25486 & 2009-01-14 & ADI &      20 &    1208 &    12.5 \\
HD 37484 & 2010-10-31 & ASDI &      45 &    2701 &  -195.2 \\
HD 38207 & 2009-03-10 & ASDI &      45 &    2701 &    15.9 \\
HD 38206 & 2008-12-18 & ADI &      20 &    1200 &     5.2 \\
HD 38206 & 2008-12-18 & ASDI &      50 &    2964 &    41.2 \\
zet Lep & 2008-12-15 & ADI &      20 &    1200 &    29.4 \\
zet Lep & 2008-12-15 & ASDI &      40 &    2432 &    34.3 \\
Beta Pic & 2008-11-22 & ASDI &      90 &    5472 &     2.3 \\
Beta Pic & 2009-12-03 & ASDI &     131 &    7964 &     2.2 \\
Beta Pic & 2009-12-03 & ASDI &     131 &    7964 &     2.2 \\
Beta Pic & 2009-12-04 & ADI &     146 &    8654 &    72.7 \\
Beta Pic & 2011-09-13 & ASDI &      81 &    4801 &     1.1 \\
HD 40136 & 2009-02-09 & ASDI &      58 &    3331 &    86.2 \\
HD 40136 & 2009-02-11 & ADI &      20 &    1208 &     4.5 \\
HD 53143 & 2009-01-13 & ADI &      20 &    1208 &     9.8 \\
HD 53143 & 2009-01-13 & ASDI &      45 &    2479 &    19.9 \\
HD 53143 & 2010-01-05 & ADI &      20 &    1208 &     8.5 \\
HD 54341 & 2008-12-15 & ADI &      20 &    1200 &    17.0 \\
HD 54341 & 2008-12-15 & ASDI &      44 &    2641 &    48.0 \\
HD 61005 & 2009-01-13 & ASDI &      80 &    3435 &   148.4 \\
HD 61005 & 2011-04-24 & ADI &      20 &    1208 &     3.5 \\
HD 71155 & 2008-12-16 & ADI &      20 &    1200 &    15.5 \\
HD 71155 & 2008-12-16 & ASDI &      46 &    2691 &    20.2 \\
HD 71155 & 2011-05-14 & ADI &      20 &    1200 &     3.5 \\
HD 85672 & 2009-01-13 & ADI &      20 &    1208 &     5.7 \\
HD 85672 & 2009-01-13 & ASDI &      45 &    2701 &    13.7 \\
TWA 7 & 2009-02-09 & ASDI &      66 &    3962 &   125.3 \\
TWA 7 & 2009-02-11 & ADI &      20 &    1208 &     2.2 \\
TWA 7 & 2010-02-28 & ADI &      20 &    1208 &    12.0 \\
TW Hya & 2009-02-12 & ADI &      40 &    2416 &     6.3 \\
TW Hya & 2009-02-12 & ASDI &     100 &    6004 &   100.7 \\
TWA 13A & 2009-03-10 & ADI &      20 &    1208 &     3.4 \\
TWA 13A & 2009-03-10 & ASDI &      45 &    2701 &    13.1 \\
TWA 13B & 2009-03-11 & ASDI &      45 &    2701 &    14.3 \\
HD 102647 & 2009-01-18 & ASDI &      37 &    2109 &    15.1 \\
HD 102647 & 2009-01-18 & ADI &      20 &    1185 &     6.9 \\
HD 107146 & 2009-01-13 & ASDI &      75 &    3933 &    22.9 \\
HD 107146 & 2009-01-13 & ADI &      20 &    1208 &     5.2 \\
HD 107146 & 2010-04-08 & ADI &      25 &    1510 &     8.1 \\
HD 109085 & 2009-02-06 & ASDI &      45 &    2817 &    46.9 \\
HD 109085 & 2009-02-06 & ADI &      20 &    1208 &    18.9 \\
HR 4796- & 2009-01-14 & ASDI &      45 &    2821 &    25.2 \\
HR 4796- & 2009-01-14 & ADI &      20 &    1208 &    21.8 \\
HR 4796- & 2012-04-06 & ADI &      64 &    3793 &    82.4 \\
HD 110058 & 2009-01-17 & ADI &      20 &    1208 &    14.8 \\
HD 110058 & 2009-01-17 & ASDI &      45 &    2701 &    26.1 \\
HD 110058 & 2012-03-28 & ADI &      20 &    1208 &    15.0 \\
HD 110411 & 2009-02-07 & ASDI &      45 &    2513 &    16.8 \\
HD 110411 & 2009-02-07 & ADI &      20 &    1208 &     7.5 \\
HD 131835 & 2009-02-12 & ASDI &      52 &    3122 &    35.0 \\
HD 131835 & 2009-04-10 & ADI &      45 &    2718 &     9.1 \\
HD 138965 & 2009-02-12 & ASDI &      68 &    4702 &    31.5 \\
HD 139664 & 2009-02-06 & ASDI &      42 &    2633 &    17.0 \\
HD 139664 & 2010-05-08 & ASDI &      46 &    2884 &     7.9 \\
HD 139664 & 2010-05-09 & ADI &      20 &    1208 &    14.3 \\
HD 141569 & 2009-03-07 & ADI &      20 &    1208 &    10.6 \\
HD 141569 & 2009-03-07 & ASDI &      65 &    3902 &    25.1 \\
HD 141569 & 2010-04-08 & ASDI &      45 &    2701 &    23.6 \\
HD 141569 & 2011-05-03 & ASDI &     114 &    6844 &    58.7 \\
HD 157728 & 2011-05-16 & ADI &      20 &    1208 &     6.3 \\
HD 157728 & 2011-05-16 & ASDI &      45 &    2736 &    14.1 \\
HIP 85340 & 2009-04-13 & ASDI &      50 &    3040 &  -319.7 \\
gamma Oph & 2009-04-08 & ASDI &      45 &    2736 &    20.0 \\
gamma Oph & 2009-04-08 & ADI &      20 &    1185 &     5.9 \\
gamma Oph & 2010-04-08 & ADI &      20 &    1185 &     6.4 \\
HD 170773 & 2011-05-12 & ASDI &      44 &    2675 &     5.0 \\
HD 170773 & 2011-10-16 & ADI &      20 &    1208 &     4.9 \\
HD 170773 & 2012-04-06 & ADI &      20 &    1208 &     3.4 \\
HD 172555 & 2009-04-09 & ADI &      20 &    1208 &     6.8 \\
HD 172555 & 2009-04-09 & ASDI &      47 &    2786 &    22.0 \\
HD 176638 & 2011-05-12 & ASDI &      45 &    2667 &    32.4 \\
HD 176638 & 2011-10-17 & ADI &      16 &     966 &     4.6 \\
HD 176638 & 2012-04-06 & ADI &      20 &    1208 &     3.9 \\
HR 7329 & 2009-04-11 & ADI &      20 &    1208 &     8.1 \\
HR 7329 & 2009-04-11 & ASDI &      45 &    2565 &    22.4 \\
HIP 95270 & 2009-04-13 & ADI &      20 &    1208 &     7.9 \\
HIP 95270 & 2009-04-13 & ASDI &      44 &    2658 &    29.2 \\
HD 182681 & 2010-08-29 & ADI &      20 &    1208 &     3.3 \\
HD 191089 & 2010-05-11 & ASDI &      45 &    2718 &  -311.3 \\
HD 191089 & 2010-05-11 & ADI &      20 &    1208 &    73.1 \\
HD 192758 & 2011-05-12 & ASDI &      45 &    2667 &    25.5 \\
HD 196544 & 2009-04-26 & ADI &      20 &    1208 &     5.0 \\
HD 196544 & 2009-04-27 & ASDI &      65 &    3952 &     5.2 \\
HD 196544 & 2010-10-31 & ASDI &      20 &    1216 &     5.4 \\
HD 196544 & 2011-04-25 & ADI &      30 &    1812 &     9.9 \\
GJ 803 & 2010-05-09 & ASDI &      59 &    3609 &    60.4 \\
GJ 803 & 2010-08-28 & ADI &      53 &    3021 &    36.9 \\
HD 206893 & 2011-10-30 & ADI &      40 &    2416 &    32.9 \\
alf PsA & 2008-11-17 & ASDI &      77 &    5149 &     6.3 \\
alf PsA & 2009-12-04 & ASDI &      99 &    5868 &     7.0 \\
alf PsA & 2009-12-04 & ADI &      99 &    5868 &     6.9 \\
alf PsA & 2011-10-17 & ASDI &      80 &    4864 &   181.9 \\
\enddata
\label{tab:obs}
\end{deluxetable}


==> table.tex <==
\begin{deluxetable}{lrrrcrrrr}
\tabletypesize{\scriptsize}
\tablecaption{Debris Disk Stars Observed by Campaign.}
\tablewidth{0pt}
\tablehead{ \colhead{Target} &\colhead{R.A.} & \colhead{Dec.} & \colhead{Distance(pc)} & \colhead{Sp.\ Type}&\colhead{Age(Myr)} & \colhead{V(mag)} & \colhead{H(mag)} & \colhead{K(mag)}}
\startdata
49 Cet  & 01 34 37.77 & $-$15 40 34.9 & 61.0 & A1V & 12 & 5.62 & 5.53 & 5.46 \\
HD 10939  & 01 46 06.27 & $-$53 31 19.5 & 57.0 & A1V & 200 & 5.00 & 5.03 & 4.96 \\
HD 15115  & 02 26 16.25 & +06 17 33.1 & 45.0 & F2 & 12 & 6.79 & 5.86 & 5.82 \\
HIP 10679  & 02 17 24.7 & +28 44 31 & 34.0 & G2 & 12 & 7.80 & 6.36 & 6.26 \\
HD 15115  & 02 26 16.2 & +06 17 33 & 45.0 & F4 & 12 & 6.79 & 5.81 & 5.77 \\
HD 17848  & 02 49 01.52 & $-$62 48 23.4 & 50.7 & A2V & 100 & 5.30 & 5.16 & 4.97 \\
HD 19668  & 03 09 42.29 & $-$09 34 46.59 & 40.2 & G0 & 70 & 8.48 & 6.79 & 6.70 \\
HD 21997  & 03 31 53.65 & $-$25 36 51.0 & 74.0 & A3IV/V & 20 & 6.38 & 6.11 & 6.10 \\
HD 22049  & 03 32 55.91 & $-$09 27 29.9 & 3.2 & K2V & 730 & 3.70 & 1.88 & 1.78 \\
HD 24966  & 03 56 29.39 & $-$38 57 43.7 & 104.0 & A0V & 10 & 6.89 & 6.87 & 6.86 \\
HD 25457  & 04 02 36.75 & $-$00 16 07.9 & 19.0 & F5V & 30 & 5.38 & 4.34 & 4.18 \\
HD 27290  & 04 16 01.59 & $-$51 29 12.0 & 20.3 & F4III & 300 & 4.30 & 3.47 & 3.51 \\
HD 31295  & 04 54 53.72 & +10 09 03.0 & 37.0 & A0V & 100 & 4.60 & 4.52 & 4.42 \\
HD 32297  & 05 02 27.43 & +07 27 39.7 & 112.0 & A0 & 30 & 8.13 & 7.62 & 7.59 \\
HIP 25486  & 05 27 04.8 & $-$11 54 04 & 26.8 & F7 & 12 & 6.30 & 5.09 & 4.93 \\
HD 37484  & 05 37 39.63 & $-$28 37 34.6 & 60.0 & F3V & 30 & 7.26 & 6.29 & 6.28 \\
HD 38207  & 05 43 20.95 & $-$20 11 21.4 & 103.0 & F2V & 20 & 8.47 & 7.55 & 7.49 \\
HD 38206  & 05 43 21.66 & $-$18 33 26.8 & 69.0 & A0V & 20 & 5.73 & 5.84 & 5.78 \\
$\zeta$ Lep  & 05 46 57.35 & $-$14 49 18.9 & 22.0 & A2VANN & 100 & 3.55 & 3.31 & 3.29 \\
$\beta$ Pic  & 05 47 17.08 & $-$51 03 59.5 & 19.0 & A3V & 12 & 3.85 & 3.54 & 3.53 \\
HD 40136  & 05 56 24.30 & $-$14 10 03.7 & 15.0 & F1V & 300 & 3.70 & 2.98 & 2.99 \\
HD 53143  & 06 59 59.67 & $-$61 20 10.6 & 18.0 & K0IV/V & 300 & 6.81 & 5.10 & 4.99 \\
HD 54341  & 07 06 20.93 & $-$43 36 38.6 & 93.0 & A0V & 10 & 6.52 & 6.48 & 6.48 \\
HD 61005  & 07 35 47.47 & $-$32 12 14.2 & 34.5 & G3/G5V & 100 & 8.20 & 6.58 & 6.46 \\
HD 71155  & 08 25 39.64 & $-$03 54 23.1 & 38.3 & A0V & 100 & 3.90 & 4.09 & 4.08 \\
HD 85672  & 09 53 59.16 & +27 41 43.5 & 93.0 & A0 & 30 & 7.59 & 7.20 & 7.19 \\
TWA 7  & 10 42 30.1 & $-$33 40 16 & 28.0 & M2 & 10 & 11.65 & 7.74 & 7.54 \\
HD 92945  & 10 43 28.28 & $-$29 03 51.4 & 22.0 & K1V & 100 & 7.72 & 5.77 & 5.66 \\
TW Hya  & 11 01 51.92 & $-$34 42 17.0 & 56.4 & K8VE & 8 & 1.10 & 7.56 & 7.30 \\
TWA 13A  & 11 21 17.2 & $-$34 46 46 & 55.0 & M1 & 10 & 11.46 & 7.77 & 7.59 \\
TWA 13B  & 11 21 17.4 & $-$34 46 50 & 55.0 & M1 & 10 & 11.96 & 8.27 & 8.09 \\
HD 102647  & 11 49 03.66 & +14 34 19.8 & 11.1 & A3VVAR & 50 & 2.10 & 1.92 & 1.88 \\
HD 107146  & 12 19 06.51 & +16 32 54.2 & 29.0 & G2V & 100 & 7.04 & 5.61 & 5.54 \\
$\eta$ Corvis & 12 32 04.25 & $-$16 11 45.5 & 18.2 & F2V & 300 & 4.30 & 3.37 & 3.37 \\
HR 4796A  & 12 36 01.03 & $-$39 52 10.2 & 67.0 & A0V & 8 & 5.78 & 5.79 & 5.77 \\
HD 110058  & 12 39 46.20 & $-$49 11 55.4 & 100.0 & A0V & 50 & 7.99 & 7.59 & 7.58 \\
HD 110411  & 12 41 53.05 & +10 14 08.3 & 36.9 & A0V & 100 & 4.90 & 4.76 & 4.68 \\
HD 131835  & 14 56 54.48 & $-$35 41 43.7 & 111.0 & A2IV & 17 & 7.88 & 7.56 & 7.52 \\
HD 138965  & 15 40 11.55 & $-$70 13 40.3 & 77.3 & A5V & 20 & 6.40 & 6.34 & 6.27 \\
HD 139664  & 15 41 11.39 & $-$44 39 40.1 & 17.5 & F5IV-V & 200 & 4.60 & 3.73 & 3.80 \\
HD 141569  & 15 49 57.76 & $-$03 55 16.2 & 99.0 & B9 & 5 & 7.10 & 6.86 & 6.82 \\
HD 157728  & 17 24 06.59 & +22 57 37.2 & 43.0 & F0IV & 100 & 5.70 & 5.22 & 5.18 \\
HIP 85340  & 17 26 22.216 & $-$24 10 31.11 & 25.7 & A3 & 324 & 4.16 & 3.96 & 3.95 \\
$\gamma$ Oph  & 17 47 53.56 & +02 42 26.2 & 29.1 & A0V & 200 & 3.70 & 3.66 & 3.62 \\
HD 170773  & 18 33 00.91 & $-$39 53 31.3 & 36.0 & F5V & 200 & 6.22 & 5.28 & 5.20 \\
HD 172555  & 18 45 26.91 & $-$64 52 16.5 & 29.0 & A7V & 12 & 4.78 & 4.25 & 4.30 \\
PZ Tel  & 18 53 05.9 & $-$50 10 50 & 49.7 & K0 & 12 & 8.42 & 6.49 & 6.37 \\
HD 176638  & 19 03 06.88 & $-$42 05 42.3 & 56.3 & A0VN & 200 & 4.70 & 4.96 & 4.75 \\
HD 181296  & 19 22 51.22 & $-$54 25 26.3 & 48.0 & A0VN & 12 & 5.03 & 5.15 & 5.01 \\
HD 181327  & 19 22 58.95 & $-$54 32 17.1 & 51.0 & F5/F6V & 12 & 7.04 & 5.98 & 5.91 \\
HD 182681  & 19 26 56.48 & $-$29 44 35.5 & 69.0 & B8/B9V & 50 & 5.66 & 5.66 & 5.68 \\
HD 191089  & 20 09 05.22 & $-$26 13 26.5 & 54.0 & F5V & 12 & 7.18 & 6.09 & 6.08 \\
HD 192758  & 20 18 15.79 & $-$42 51 36.2 & 62.0 & F0V & 40 & 7.02 & 6.30 & 6.21 \\
HD 196544  & 20 37 49.13 & +11 22 39.7 & 54.3 & A2V & 30 & 5.40 & 5.37 & 5.30 \\
AU Mic  & 20 45 09.49 & $-$31 20 26.7 & 10.0 & M1Ve & 12 & 8.81 & 4.83 & 4.53 \\
HD 206893  & 21 45 21.91 & $-$12 47 00.0 & 39.0 & F5V & 200 & 6.69 & 5.69 & 5.59 \\
Fomalhaut  & 22 57 39.02 & $-$29 37 19.4 & 7.7 & A3V & 220 & 1.20 & 0.94 & 0.94 \\
\enddata
\label{tab:obs}
\end{deluxetable}


==> tableb.tex <==
\begin{deluxetable}{lrrrcrrrr}
\tabletypesize{\scriptsize}
\tablecaption{Debris Disk Stars Observed by Campaign.}
\tablewidth{0pt}
\tablehead{ \colhead{Target} &\colhead{R.A.} & \colhead{Dec.} & \colhead{Distance(pc)} & \colhead{Sp.\ Type}&\colhead{Age(Myr)} & \colhead{V(mag)} & \colhead{H(mag)} & \colhead{K(mag)}}
\startdata
49 Cet  & 01 34 37.77 & $-$15 40 34.9 & 61.0 & A1V & 12 & 5.62 & 5.53 & 5.46 \\
HD 10939  & 01:46:06.27 & $-$53:31:19.50 & 57.0 & A1 & 200 & 5.00 & 5.03 & 4.96 \\
HD 15115  & 02 26 16.25 & +06 17 33.1 & 45.0 & F2 & 12 & 6.79 & 5.86 & 5.82 \\
HIP 10679  & 02:17:24.7 & +28:44:31 & 34.0 & G2 & 12 & 7.80 & 6.36 & 6.26 \\
HD 15115  & 02:26:16.2 & +06:17:33 & 45.0 & F4 & 12 & 6.79 & 5.81 & 5.77 \\
HD 17848  & 02:49:01.52 & $-$62:48:23.40 & 50.7 & A2 & 100 & 5.30 & 5.16 & 4.97 \\
HD 19668  & 03:09:42.29 & $-$09:34:46.59 & 40.2 & G0 & 70 & 8.48 & 6.79 & 6.70 \\
HD 21997  & 03 31 53.65 & $-$25 36 51.0 & 74.0 & A3IV/V & 20 & 6.38 & 6.11 & 6.10 \\
HD 22049  & 03 32 55.91 & $-$09 27 29.9 & 3.2 & K2V & 730 & 3.70 & 1.88 & 1.78 \\
HD 24966  & 03 56 29.39 & $-$38 57 43.7 & 104.0 & A0V & 10 & 6.89 & 6.87 & 6.86 \\
HD 25457  & 04:02:36.7449 & $-$00:16:08.123 & 19.2 & F5 & 70 & 5.38 & 4.34 & 4.28 \\
HD 27290  & 04:16:01.59 & $-$51:29:12.00 & 20.3 & F4 & 300 & 4.30 & 3.47 & 3.51 \\
HD 31295  & 04 54 53.72 & +10 09 03.0 & 37.0 & A0V & 100 & 4.60 & 4.52 & 4.42 \\
HD 32297  & 05:02:27.43 & +07:27:39.70 & 112.0 & A0 & 30 & 8.13 & 7.62 & 7.59 \\
HIP 25486  & 05:27:04.8 & $-$11:54:04 & 26.8 & F7 & 12 & 6.30 & 5.09 & 4.93 \\
HD 37484  & 05:37:39.63 & $-$28:37:34.60 & 60.0 & F3 & 30 & 7.26 & 6.29 & 6.28 \\
HD 38207  & 05:43:20.95 & $-$20:11:21.40 & 103.0 & F2 & 20 & 8.47 & 7.55 & 7.49 \\
HD 38206  & 05:43:21.66 & $-$18:33:26.80 & 69.0 & A0 & 20 & 5.73 & 5.84 & 5.78 \\
$\zeta$ Lep  & 05:46:57.35 & $-$14:49:18.90 & 22.0 & A2 & 100 & 3.55 & 3.31 & 3.29 \\
$\beta$ Pic  & 05:47:17.1 & $-$51:03:59 & 19.3 & A5 & 12 & 3.90 & 3.54 & 3.53 \\
HD 40136  & 05:56:24.30 & $-$14:10:03.70 & 15.0 & F1 & 300 & 3.70 & 2.98 & 2.99 \\
HD 53143  & 06:59:59.67 & $-$61:20:10.60 & 18.0 & K0 & 300 & 6.81 & 5.10 & 4.99 \\
HD 54341  & 07:06:20.93 & $-$43:36:38.60 & 93.0 & A0 & 10 & 6.52 & 6.48 & 6.48 \\
HD 61005  & 07:35:47.47 & $-$32:12:14.20 & 34.5 & G3 & 100 & 8.20 & 6.58 & 6.46 \\
HD 71155  & 08:25:39.64 & $-$03:54:23.10 & 38.3 & A0 & 100 & 3.90 & 4.09 & 4.08 \\
HD 85672  & 09:53:59.16 & +27:41:43.50 & 93.0 & A0 & 30 & 7.59 & 7.20 & 7.19 \\
TWA 7  & 10:42:30.1 & $-$33:40:16 & 28.0 & M2 & 10 & 11.65 & 7.74 & 7.54 \\
HD 92945  & 10:43:28.3 & $-$29:03:51.4 & 21.6 & K1 & 70 & 7.76 & 5.77 & 5.69 \\
TW Hya  & 11:01:52.0 & $-$34:42:17 & 56.4 & K7 & 10 & 10.80 & 7.56 & 7.30 \\
TWA 13A  & 11:21:17.2 & $-$34:46:46 & 55.0 & M1 & 10 & 11.46 & 7.77 & 7.59 \\
TWA 13B  & 11:21:17.4 & $-$34:46:50 & 55.0 & M1 & 10 & 11.96 & 8.27 & 8.09 \\
HD 102647  & 11:49:03.66 & +14:34:19.80 & 11.1 & A3 & 50 & 2.10 & 1.92 & 1.88 \\
HD 107146  & 12:19:06.5015 & +16:32:53.869 & 28.5 & G2 & 185 & 7.07 & 5.61 & 5.61 \\
HD 109085  & 12:32:04.2270 & $-$16:11:45.627 & 18.2 & F2 & 100 & 4.31 & 3.37 & 3.46 \\
HR 4796 A  & 12:36:01.2 & $-$39:52:10 & 67.1 & A0 & 10 & 5.80 & 5.79 & 5.77 \\
HD 110058  & 12:39:46.20 & $-$49:11:55.40 & 100.0 & A0 & 50 & 7.99 & 7.59 & 7.58 \\
HD 110411  & 12:41:53.05 & +10:14:08.30 & 36.9 & A0 & 100 & 4.90 & 4.76 & 4.68 \\
HD 131835  & 14:56:54.48 & $-$35:41:43.70 & 111.0 & A2 & 17 & 7.88 & 7.56 & 7.52 \\
HD 138965  & 15:40:11.55 & $-$70:13:40.30 & 77.3 & A5 & 20 & 6.40 & 6.34 & 6.27 \\
HD 139664  & 15:41:11.38 & $-$44:39:40.34 & 17.5 & F5 & 200 & 4.64 & 3.73 & 3.80 \\
HD 141569  & 15:49:57.76 & $-$03:55:16.20 & 99.0 & B9 & 5 & 7.10 & 6.86 & 6.82 \\
HD 157728  & 17:24:06.59 & +22:57:37.20 & 43.0 & F0 & 100 & 5.70 & 5.22 & 5.18 \\
HIP 85340  & 17:26:22.216 & $-$24:10:31.11 & 25.7 & A3 & 324 & 4.16 & 3.96 & 3.95 \\
$\gamma$ Oph  & 17:47:53.56 & +02:42:26.20 & 29.1 & A0 & 200 & 3.70 & 3.66 & 3.62 \\
HD 170773  & 18:33:00.91 & $-$39:53:31.30 & 36.0 & F5 & 200 & 6.22 & 5.28 & 5.20 \\
HD 172555 A  & 18:45:26.9 & $-$64:52:16.5 & 29.2 & A5 & 12 & 4.80 & 4.25 & 4.42 \\
PZ Tel  & 18:53:05.9 & $-$50:10:50 & 49.7 & K0 & 12 & 8.42 & 6.49 & 6.37 \\
HD 176638  & 19:03:06.88 & $-$42:05:42.30 & 56.3 & A0 & 200 & 4.70 & 4.96 & 4.75 \\
HD 181296  & 19 22 51.22 & $-$54 25 26.3 & 48.0 & A0VN & 12 & 5.03 & 5.15 & 5.01 \\
HD 181327  & 19 22 58.95 & $-$54 32 17.1 & 51.0 & F5/F6V & 12 & 7.04 & 5.98 & 5.91 \\
HD 182681  & 19:26:56.48 & $-$29:44:35.50 & 69.0 & B8 & 50 & 5.66 & 5.66 & 5.68 \\
HD 191089  & 20:09:05.2 & $-$26:13:27 & 53.0 & F5 & 12 & 7.18 & 6.12 & 6.08 \\
HD 192758  & 20:18:15.79 & $-$42:51:36.20 & 62.0 & F0 & 40 & 7.02 & 6.30 & 6.21 \\
HD 196544  & 20:37:49.13 & +11:22:39.70 & 54.3 & A2 & 30 & 5.40 & 5.37 & 5.30 \\
GJ 803  & 20:45:09.5 & $-$31:20:27.1 & 9.9 & M0 & 12 & 8.81 & 4.83 & 5.16 \\
HD 206893  & 21:45:21.91 & $-$12:47:00.00 & 39.0 & F5 & 200 & 6.69 & 5.69 & 5.59 \\
Fomalhaut  & 22:57:39.02 & $-$29:37:19.40 & 7.7 & A3 & 220 & 1.20 & 0.94 & 0.94 \\
\enddata
\label{tab:obs}
\end{deluxetable}

